Improving Text-based Person Search via Part-level Cross-modal Correspondence

Text-based person search is the task of finding person images that are the most relevant to the natural language text description given as query. The main challenge of this task is a large gap between the target images and text queries, which makes it difficult to establish correspondence and distinguish subtle differences across people. To address this challenge, we introduce an efficient encoder-decoder model that extracts coarse-to-fine embedding vectors which are semantically aligned across the two modalities without supervision for the alignment. There is another challenge of learning to capture fine-grained information with only person IDs as supervision, where similar body parts of different individuals are considered different due to the lack of part-level supervision. To tackle this, we propose a novel ranking loss, dubbed commonality-based margin ranking loss, which quantifies the degree of commonality of each body part and reflects it during the learning of fine-grained body part details. As a consequence, it enables our method to achieve the best records on three public benchmarks.

==> figures/fig_encoder_decoder.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/CVPR24_encoder_decoder.pdf}
    \vspace{-1mm}   
    \caption{Details of encoder-decoder architecture.}
    \label{fig:encoder_decoder}
\end{figure}

==> figures/fig_qual_icfg.tex <==
%\setcounter{figure}{0} 
%\counterwithin{figure}{section}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/SIGIR_qualitative_ICFG.pdf}
    %\vspace{-2mm}
    \caption{
    Qualitative results of our method on the ICFG-PEDES dataset. 
    Query texts and the top-5 retrieval results of our method are presented, 
    The true and false matches are colored green and red, respectively.
    }
    \label{fig:qual_icfg}
\end{figure*}

% \begin{figure*}[t!]
%     \centering
%     % \includegraphics[width=0.75\textwidth]{Supp_figures/ICCV23_supp_qualitative_CUHK.pdf}
%     \includegraphics[width=0.88\textwidth]{figures/ICCV23_qualitative_CUHK_v2.pdf}
%     \vspace{-2mm}
%     \caption{
%     Qualitative results of our method on the CUHK-PEDES dataset. 
%     Query texts and the top-5 retrieval results of our method are presented, 
%     The true and false matches are colored green and red, respectively.
%     }
%     \label{fig:qual_cuhk}
% \end{figure*}

% \newpage
% \begin{figure*}[t!]
%     \centering
%     % \includegraphics[width=0.80\textwidth]{Supp_figures/ICCV23_qualitative_ICFG.pdf}
%     \includegraphics[width=0.90\textwidth]{figures/ICCV23_qualitative_ICFG_v2.pdf}
%     \vspace{-2mm}
%     \caption{
%     Qualitative results of our method on the ICFG-PEDES dataset. 
%     Query texts and the top-5 retrieval results of our method are presented, 
%     The true and false matches are colored green and red, respectively.
%     }
%     \label{fig:qual_icfg}
% \end{figure*}

% \newpage
% \begin{figure*}[t!]
%     \centering
%     % \includegraphics[width=0.80\textwidth]{Supp_figures/ICCV23_qualitative_ICFG.pdf}
%     \includegraphics[width=0.90\textwidth]{figures/ICCV23_qualitative_RSTP.pdf}
%     \vspace{-2mm}
%     \caption{
%     Qualitative results of our method on the RSTPReid dataset. 
%     Query texts and the top-5 retrieval results of our method are presented, 
%     The true and false matches are colored green and red, respectively.
%     }
%     \label{fig:qual_rstp}
% \end{figure*}

==> figures/fig_qual_rstp.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/SIGIR_qualitative_RSTP.pdf}
    %\vspace{-2mm}
    \caption{
    Qualitative results of our method on the RSTPReid dataset. 
    Query texts and the top-5 retrieval results of our method are presented, 
    The true and false matches are colored green and red, respectively.
    }
    \label{fig:qual_rstp}
\end{figure*}
